Encoder-Decoder Architecture for Supervised Dynamic Graph Learning: A Survey

In recent years, the prevalent online services generate a sheer volume of user activity data. Service providers collect these data in order to perform client behavior analysis, and offer better and more customized services. Majority of these data can be modeled and stored as graph, such as the social graph in Facebook, user-video interaction graph in Youtube. These graphs need to evolve over time to capture the dynamics in the real world, leading to the invention of dynamic graphs. However, the temporal information embedded in the dynamic graphs brings new challenges in analyzing and deploying them. Events staleness, temporal information learning and explicit time dimension usage are some example challenges in dynamic graph learning. In order to offer a convenient reference to both the industry and academia, this survey presents the Three Stages Recurrent Temporal Learning Framework based on dynamic graph evolution theories, so as to interpret the learning of temporal information with a generalized framework. Under this framework, this survey categories and reviews different learnable encoder-decoder architectures for supervised dynamic graph learning. We believe that this survey could supply useful guidelines to researchers and engineers in finding suitable graph structures for their dynamic learning tasks.

==> IRDG/regular_graph.tex <==

One critical factor to consider when applying supervised dynamic graph learning algorithms is whether the given dynamic graph would have change in its nodes over time, namely adding or dropping nodes.   
Therefore, in this review we propose a new way to categorize dynamic graph based on whether it has change in its nodes' identity over time. 

\begin{defn} 
\textbf{Regular Dynamic Graph(RDG)}: a dynamic graph $G_T(V_T,E_T)$ is regular if $V_{t_i} = V_{t_j} \forall t_i ,t_j \in T \wedge t_i \neq t_j$, 
\end{defn}

\begin{defn} 
\textbf{Irregular Dynamic Graph(IRDG)}: a dynamic graph $G_t(V_t,E_t)$ is irregular if $\exists i, j: V_i \neq V_j C \wedge i\neq j$.
\end{defn}


Some algorithms assume that the input dynamic graph is regular while others not.
ST-GCN\cite{yan2018spatial} assumes the input dynamic graph has no change in nodes, since it is proposed for pattern detection in video streams and the dimension of the stream will be the same frame after frame.
And TGN\cite{rossi2020temporal} is proposed to addressed the challenge of change in nodes over time.
Algorithms assuming the input to be an RDG requires a retrain if the target graph has change in nodes when performing extrapolation tasks and hence is not appropriate in real world application especially for large scale dynamic graphs for which model training is very expensive.

In this survey, we observe two main ideas from the reviewed algorithms.
These ideas enable learning in IRDG.

\subsection{Weight Sharing Between Nodes}
To make a learning model adaptable to IRDG, the trainable weights in the model has to be shared between nodes.
Otherwise, if the trainable weight is unique to nodes or edges, such as in shallow static graph embedding based encoders and the TPP based decoder such as the one in Know-Evolve\cite{trivedi2017know}, the learning model is not adaptable to IRDG.
If weights are shared between nodes and just unique to features, then the learning model could perform learning tasks for new added nodes without retraining as long as they have the same set of features.
Moreover, weight sharing is able to speed up the training process as well as to enable semi-supervised learning tasks.
However, with only weight sharing, the learning model cannot capture the input dynamic graph's global connectivity information.

\subsection{Iterative Message Passing}
The traditional way to learn a graph's global connectivity information is by matrix factorization on the adjacency matrix or random walk. 
However these methods can only work with non-attributed graph and serve as static graph encoder.
GraphSAGE\cite{hamilton2017inductive} is proposed to generate graph embedding inductively to learn from both graph attributes and global connectivity. 
By learning inductively, it actually performs iterative message passing neighborhood aggregation until the resulting embedding converges to a stable value.
Such that, when serving as static graph encoder, it does not require model training and hence can be used as the encoder in supervised IRDG learning. 
Practitioners only needs to train the weight sharing sequential decoder, and the combination could learn the temporal dynamic from graph attribute and global connectivity for RDG and IRDG as well.   






